Cross-lingual Supervision Improves Unsupervised Neural Machine Translation

Neural machine translation~(NMT) is ineffective for zero-resource languages. Recent works exploring the possibility of unsupervised neural machine translation (UNMT) with only monolingual data can achieve promising results. However, there are still big gaps between UNMT and NMT with parallel supervision. In this work, we introduce a multilingual unsupervised NMT (\method) framework to leverage weakly supervised signals from high-resource language pairs to zero-resource translation directions. More specifically, for unsupervised language pairs \texttt{En-De}, we can make full use of the information from parallel dataset \texttt{En-Fr} to jointly train the unsupervised translation directions all in one model. \method is based on multilingual models which require no changes to the standard unsupervised NMT. Empirical results demonstrate that \method significantly improves the translation quality by more than 3 BLEU score on six benchmark unsupervised translation directions.

==> 035background.tex <==
%\subsection{Background: Multilingual NMT \& UNMT}

% \begin{figure*}[htb]
% \centering
% \includegraphics[width=0.95\textwidth]{m.pdf}
% \caption{The framework of our model.}
% \label{fig:mo}
% \end{figure*}
\paragraph{Multilingual NMT}
Neural Machine Translation, which is a sequence to sequence model consisting of an encoder and decoder, can have the following building blocks: RNNs~\cite{sutskever_nips2014_s2smt}, CNNs~\cite{gehring2017cnnmt}, and Transformer~\cite{vaswani2017transformer}.
NMT model encodes input sentences to intermediate representations and then decodes the target sentences word by word.

Formally, $x_i$ denotes a sentence in language $L_i$.
For supervised machine translation models, given parallel dataset $D_{s,t}$ with source language $L_s$ and target language $L_t$, we use $\mathcal{L}_{s\to t}$ to denote the supervised training procedure from language $L_s$ to language $L_t$. The training loss for a single sentence can be defined as:
\begin{equation}
\lst = \mathbb{E}_{(x_s,x_t)\sim D_{s,t}} [-\log P(x_t|x_s)].
\label{eq:mt}
\end{equation}

In an effort to extend the individual NMT to a multilingual NMT model, \citet{johnson-etal-2017-googlemnmt} proposed to train multiple translation directions all in one model, which results in the loss being defined as:
\[
\mathcal{L}^{mul} = \sum_{(s,t)\in \mathcal{E}} \lst,
\]
where $\mathcal{E}$ indicates all translation directions with parallel data.
The training and architecture are extremely simple without large model modification. Benefiting from the shared architecture, the multilingual model can even translate zero-shot directions.

\paragraph{Unsupervised NMT}
For unsupervised machine translation systems, only monolingual data is utilized during training.
This method heavily relies on the dual structure of machine translations.
Due to the ill-posed nature, it is important to find a way to associate the source side languages and the target side languages, the methods for which include word embedding alignment~\cite{artetxe-2017-unsupword,artetxe2018unsupervisedmt,lample2018unsupword,lample2018unsupervisedmt}, joint learning of embeddings~\cite{lample-2018-pbumt} and pre-training language models~\cite{lample2019cross,song2019icml-mass}.
This step can also be seen as a good initialization of the system.
The observation that a better start will result in a much easier optimization of UNMT and deliver better results is in line with the our target.

After the initialization, the unsupervised neural machine translation systems use language modeling via denoising auto-encoders and iterative back-translation to train the model.
Language model gives a prior about how to encode and generate sentences in one language.
Adding noise to the model prevents the system from only copying and improves the quality of translation.



After that, we can use these data to train the model with supervised method from $L_s$ to $L_t$.
We use $\mathcal{B}_{s\to t}$ to denote this back translation procedure.
Back-translation is the key part in the unsupervised setting to connects the two languages and trains the model in the way similar to the supervised one.
For an unsupervised machine translation system with two languages $L_s, L_t$, and monolingual datasets $D_s, D_t$, the losses of the two steps respectively are:

\begin{equation}
\begin{split}
\mathcal{L}_{\mathcal{B}_{t\to s}} = &\mathbb{E}_{x_s\sim D_s} [-\log P(x_s|u_t(x_s)], \\
\mathcal{L}_{\mathcal{B}_{s\to t}} = &\mathbb{E}_{x_t\sim D_t} [-\log P(x_t|u_1(x_t)],
\end{split}
\label{eq:bt}
\end{equation}

where $C$ is a noise model to randomly drop, swap or blank some words, and $u_i(x_j)$ denotes the sentence in language $L_i$ inferred from the sentence in language $L_j$ with the same model.
Then the total loss of an unsupervised machine translation is:
\[
\lus = \lambda_l (\mathcal{L}_{\mathcal{LM}_{1}} + \mathcal{L}_{\mathcal{LM}_{2}}) +
\lambda_b (\mathcal{L}_{\mathcal{BT}_{2\to 1}} + \mathcal{L}_{\mathcal{BT}_{1\to 2}}),
\]
where $\lambda_l$ and $\lambda_b$ are coefficients.
During training, $\lambda_l$ is gradually reduced to 0.
If the system is initialized with pre-training language models, $\lambda_l$ can be even set to 0.
The initialization and back-translation are the most important parts of unsupervised machine translation.

Furthermore, there is an assumption for unsupervised machine translation that latent representations for different languages need to be in the shared latent space.
Since only monolingual data is available, shared representations ensure that the model has connections of these languages.
It is only on this basis that back translation can be properly carried out.
Sharing the model is one of the simplest ways to satisfy this assumption.
